Energy- and momentum-resolved Cooper-pair emission from a cuprate superconductor

Superconductivity arises from Cooper pairing, but conventional photoemission probes electrons individually rather than as pairs. Here we report the observation of Cooper-pair emission from an optimally doped cuprate superconductor using two-electron angle-resolved photoemission (2e-ARPES). Below the superconducting transition, we observe a distinct two-electron emission peak at zero pair binding energy and zero pair momentum that disappears in the normal state, revealing the characteristic fingerprint of a Cooper pair. Unexpectedly, the joint energy distribution broadens markedly along the relative-energy axis as temperature decreases, while the total energy width remains nearly unchanged. This anomalous behavior cannot be explained by instrumental resolution, static disorder or thermal broadening, and instead points to scattering processes involving collective excitations of the superconductor. Our results establish 2e-ARPES as a probe of both Cooper-pair emission and the many-body dynamics of the superconducting state.

==> arxiv_main.tex <==
\makeatletter
\let\oldaddcontentsline\addcontentsline
\renewcommand{\addcontentsline}[3]{}

\input{main_body}

\let\addcontentsline\oldaddcontentsline
\makeatother

\makeatletter
\bibliographystyle@latex{naturemag}
\makeatother
\bibliography{bib}


==> main_body.tex <==
\title{Energy- and momentum-resolved Cooper-pair emission from a cuprate superconductor}

\author{Henry Amir}
\thanks{These authors contributed equally to this work.}
\affiliation{Department of Physics, The Grainger College of Engineering, University of Illinois Urbana-Champaign, Urbana, Illinois 61801, USA}
\affiliation{Materials Research Laboratory, The Grainger College of Engineering, University of Illinois Urbana-Champaign, Urbana, Illinois 61801, USA}

\author{Jack Zwettler}
\thanks{These authors contributed equally to this work.}
\affiliation{Department of Physics, The Grainger College of Engineering, University of Illinois Urbana-Champaign, Urbana, Illinois 61801, USA}
\affiliation{Materials Research Laboratory, The Grainger College of Engineering, University of Illinois Urbana-Champaign, Urbana, Illinois 61801, USA}

\author{Ka Ho Wong}
\affiliation{Department of Physics, University of Illinois Chicago, Chicago, Illinois 60607, USA}

\author{Genda Gu}
\affiliation{Condensed Matter Physics and Materials Science Department, Brookhaven National Laboratory, Upton, NY 11973}

\author{Rafael M. Fernandes} 
\affiliation{Department of Physics, The Grainger College of Engineering, University of Illinois Urbana-Champaign, Urbana, Illinois 61801, USA}
\affiliation{Anthony J. Leggett Institute for Condensed Matter Theory, The Grainger College of Engineering, University of Illinois Urbana-Champaign, Urbana, Illinois 61801, USA}

\author{Jorge Noronha} 
\affiliation{Illinois Center for Advanced Studies of the Universe and Department of Physics, The Grainger College of Engineering, University of Illinois Urbana-Champaign, Urbana, Illinois 61801, USA}

\author{Dirk K.~Morr}
\affiliation{Department of Physics, University of Illinois Chicago, Chicago, Illinois 60607, USA}

\author{Fahad Mahmood}
\affiliation{Department of Physics, The Grainger College of Engineering, University of Illinois Urbana-Champaign, Urbana, Illinois 61801, USA}
\affiliation{Materials Research Laboratory, The Grainger College of Engineering, University of Illinois Urbana-Champaign, Urbana, Illinois 61801, USA}

\maketitle

\noindent\textbf{Superconductivity arises from Cooper pairing, but conventional photoemission probes electrons individually rather than as pairs. Here we report the observation of Cooper-pair emission from an optimally doped cuprate superconductor using two-electron angle-resolved photoemission (2e-ARPES). Below the superconducting transition, we observe a distinct two-electron emission peak at zero pair binding energy and zero pair momentum that disappears in the normal state, revealing the characteristic fingerprint of a Cooper pair. Unexpectedly, the joint energy distribution broadens markedly along the relative-energy axis as temperature decreases, while the total energy width remains nearly unchanged. This anomalous behavior cannot be explained by instrumental resolution, static disorder or thermal broadening, and instead points to scattering processes involving collective excitations of the superconductor. Our results establish 2e-ARPES as a probe of both Cooper-pair emission and the many-body dynamics of the superconducting state.}

\medskip

Superconductivity arises when electrons form Cooper pairs and develop long-range phase coherence \cite{BCS,Tinkham2004}. Yet, most spectroscopic probes of superconductors access only single-particle excitations. Angle-resolved photoemission spectroscopy (ARPES), scanning tunneling spectroscopy, transport, and optical measurements have established the phenomenology of several superconductors, revealing the gap structure, quasiparticle excitations, and intertwined orders \cite{Damascelli_2003,Lee2006,Norman2011,Sobota2021,Keimer2015,Fradkin2015}. However, these techniques probe superconductivity only indirectly -- they measure how individual electrons are affected by pairing, rather than directly accessing the two electrons that form a Cooper pair.

\begin{figure}
    \centering\includegraphics[width=\columnwidth]{fig1_v8.pdf}
    \caption{\textbf{Two-electron ARPES geometry} \textbf{(a)} Schematic of the two-electron angle-resolved photoemission spectroscopy (2e-ARPES) process, in which absorption of a single XUV photon leads to the coincident emission of two photoelectrons that are detected simultaneously. \textbf{(b)} Simulated 2e-ARPES joint energy distribution for Cooper-pair emission from a $d$-wave superconductor with zero pair momentum ($\mathbf{k}_1=-\mathbf{k}_2$; see lower left inset showing opposite antinodal momenta on the typical cuprate Fermi surface). Here, $P^{(2)}$ is the normalized pair-photoemission intensity (a.u.), and $E_1$ and $E_2$ are the photoelectron energies relative to the Fermi level. The condensate contribution peaks at $E_1=E_2=0$. Simulation details are provided in the Supplementary Information. }
    \label{fig:general idea}
\end{figure}

\begin{figure*}
\centering
\includegraphics[width=16.8cm]{fig2_ah_fixed.pdf}
\caption{\textbf{Single-particle ARPES characterization and calibration.} \textbf{(a)} Schematic of the momentum regions probed by single-ARPES (blue shaded regions numbered 1 and 3) and 2e-ARPES (red shaded regions 4 and 5) at a photon energy of 22.8~eV in the experimental geometry shown in Fig.~1, where the sample normal is oriented at $45^\circ$ relative to each analyzer. Region 2 is accessed by rotating the sample normal along the central axis of one analyzer (see Supplementary Information for calculations). \textbf{(b)} Constant-energy cuts near the Fermi level as measured at the center of the Brillouin zone and in regions 1 and 3 in (a). Data from regions 1 and 3 are acquired simultaneously using the two detectors, while region 2 is measured with the rotated sample geometry. An energy-and-momentum dispersive cut along the gray dotted line is shown in the top panel.} 
\label{fig:singleARPES}
\end{figure*}

That limitation is especially acute in the cuprates, in which high-$T_c$ superconductivity emerges from a strongly interacting electronic environment characterized by short coherence lengths, pronounced momentum-space anisotropy, and the presence of competing orders, all developing from a normal state that departs strongly from conventional Fermi-liquid behavior \cite{Lee2006,Abanov2003,Norman2011,Keimer2015,Fradkin2015}. In such materials, signatures observed in the single-particle spectrum do not by themselves reveal whether the underlying paired state is coherent, nor do they determine the pair momentum. A direct probe of pairing should therefore both establish whether the initial state supplies a coherent electron pair and determine the pair momentum, $\mathbf K=\mathbf k_1+\mathbf k_2$, where $\mathbf k_i$ is the measured in-plane momentum of electron $i$. For a spatially uniform, phase-coherent superconducting condensate, such a measurement should reveal a pair signal concentrated near $\mathbf K=0$, whereas weight at finite $\mathbf K$ could indicate finite-momentum pairing. Furthermore, resolving the energies of both electrons could provide access to the interactions and excitations of the material that influence the pair-emission process \cite{Daix2026}.

A promising route to such a probe is two-electron angle-resolved photoemission spectroscopy (2e-ARPES). In this approach, absorption of a high-energy photon ejects two photoelectrons whose energies, $E_1$ and $E_2$, and in-plane momenta, $\mathbf{k}_1$ and $\mathbf{k}_2$, are recorded in coincidence (Fig.~\ref{fig:general idea}a). Here, $E_i$ is measured relative to the Fermi level, and the coincidence events define the full energy- and momentum-resolved distribution $P^{(2)}(E_1,\mathbf{k}_1;E_2,\mathbf{k}_2)$. This approach builds on more than four decades of attempts at electron-coincidence double photoemission. Beginning with Auger measurements in Cu \cite{Haak1978}, one-photon double photoemission from valence states was subsequently demonstrated in Cu and Ni and extended to insulators and correlated oxides \cite{Haak1978,Herrmann1998,Schumann2007,Hattass2008,Schumann2011,Schumann2012,Chiang2020,Schumann2020}. Theoretical work predicts that a 2e-ARPES measurement of superconductors contains a contribution arising directly from the superconducting condensate and sensitive to the momentum and internal structure of Cooper pairs \cite{Berakdar1998,Berakdar2003,KOUZAKOV2007,Wong2024,Wong2025,Su_2024}. Complementary theoretical approaches have also considered two-photon, two-electron coincidence photoemission (termed pair-ARPES or correlation-ARPES) in which two separate photon-induced electron emissions are measured in coincidence to probe two-particle correlations and pairing \cite{Su2020,Devereaux2023,Kemper2025,Bonca2026}. We note that these two-photon approaches are distinct from the single-photon double-photoemission process studied here. For the latter process, the simulated condensate contribution from electrons emitted from paired states near the Fermi surface produces a pronounced peak centered at $E_1=E_2=0$ in the joint energy distribution, as illustrated in Fig.~\ref{fig:general idea}b (see Supplementary Information for simulation details). Yet, despite longstanding interest, this condensate peak associated with superconductivity has not previously been observed. The challenge is to combine a sufficiently high photoemission coincidence rate with energy resolution on the superconducting scale and momentum-selective detection near opposite points of the Fermi surface \cite{Chiang2020}.

In this work, we perform 2e-ARPES measurements on the optimally-doped cuprate superconductor Bi$_2$Sr$_2$CaCu$_2$O$_{8+\delta}$ (Bi-2212) ($T_c = 93$~K), focusing on photoelectron pairs near the antinodal regions of the Brillouin zone. Our purpose-built 2e-ARPES setup combines a high-flux, 525-kHz XUV source with better than 15-meV energy resolution, overcoming the instrumental limitations that have previously prevented the superconducting condensate peak from being resolved (Methods and \cite{Setup}). In the joint energy map $P^{(2)}(E_1,E_2)$, we observe a zero-pair-binding-energy peak that appears below $T_c$ and is absent above it, providing direct evidence for the emission of correlated electron pairs from the superconducting state. The same events are concentrated near zero pair momentum, $\mathbf K=0$. To our knowledge, this is the first momentum- and energy-resolved observation of Cooper-pair emission from a superconductor. We further find that the widths along $E_+$ and $E_-$ evolve differently. The total-energy width is nearly temperature independent, whereas the relative-energy width broadens strongly on cooling. We argue that this behavior provides insights into the correlations present inside the superconducting state.

We first characterize the electronic structure of our Bi-2212 samples using conventional ARPES. In this configuration, the sample normal is oriented at $45^\circ$ relative to each analyzer, enabling simultaneous detection of photoelectrons from opposite momentum regions of the Brillouin zone. For our photon energy of 22.8~eV, the expected momentum regions probed by conventional ARPES in this geometry are shown by the blue shaded regions 1 and 3 in Fig.~2a (See Supplementary Information for detailed calculations). The resulting constant energy cuts  near the Fermi level for each detector are shown in Fig.~2b. To further characterize the sample, we also measure the ARPES spectra around the center of the Brillouin zone (region 2 in Fig.~2a) by rotating the sample such that its surface normal is oriented along the central axis of the analyzer. Overall, the measured spectra reproduces the expected Fermi-surface of optimally doped Bi-2212 in each of the probing regions \cite{Ding1996}.      

Establishing a reliable Fermi-level reference is essential for interpreting the two-electron coincidence measurements. We therefore exploit the well-known nodal structure of the Bi-2212 pairing state, where the superconducting gap vanishes along the nodal direction \cite{Hashimoto2014,Keimer2015}. This nodal point appears at the center of a Fermi arc and provides a robust, gapless reference for energy calibration (Supplementary Information). We determine the photoelectron kinetic energy corresponding to the Fermi level by analyzing the Fermi–Dirac cutoff across this nodal Fermi edge on both detectors. This calibration establishes the Fermi-level reference, relative to which $E_1$ and $E_2$ are defined for all subsequent 2e-ARPES measurements performed with the same sample orientation, detector geometry, and experimental conditions. 

We next perform 2e-ARPES measurements using the same sample orientation and detector geometry as in the conventional ARPES measurements. The setup is configured to detect correlated pairs of photoelectrons emitted near the Fermi energy (around zero binding energy). In contrast to single-electron photoemission, the correlated pair of electrons generated by absorption of a single photon share the available kinetic energy, and therefore arrive at the detectors with substantially lower kinetic energies than electrons emitted in conventional ARPES from the same binding energy \cite{Chiang2020,Kostanovskiy2015}. As a consequence, the momentum-space region accessed in 2e-ARPES is shifted relative to the corresponding conventional ARPES measurement. The expected momentum regions probed in the two-electron measurement are shown schematically in Fig.~2a by the red shaded regions 4 and 5. These regions contain the antinodal points of the Fermi-surface of Bi-2212, thus enabling direct access to the maximum superconducting gap \cite{Mahmood2022}.

\begin{figure}
\centering
\includegraphics[width=\columnwidth]{fig3.pdf}
\caption{\textbf{2e-ARPES measurements on Bi-2212 below and above $T_c$} \textbf{(a,b)} Joint energy maps of the normalized correlation measure $P^{(2)}(E_1,E_2)$, integrated over the momentum regions shown in Fig.~2a, measured at 8.5~K and 200~K, respectively. Here, $E_1$ and $E_2$ are the photoelectron energies relative to the Fermi level. The solid and dashed arrows in (a) indicate the diagonal ($E_+=E_1+E_2$) and anti-diagonal ($E_-=E_1-E_2$) directions, respectively. \textbf{(c)} Cuts along the diagonal ($E_+$) direction in (a) and (b). Cuts along the anti-diagonal ($E_-$) direction are shown in Fig.~4. Shaded regions around the curves represent the 68\% confidence interval calculated from bootstrap resampling (see Methods and Supplementary Information). \textbf{(d)} Pair-momentum distribution constructed from coincidence events within an approximately $75~\mathrm{meV}\times75~\mathrm{meV}$ energy window centered at $E_1=E_2=0$ in (a).} 
\label{fig:2eARPES}
\end{figure}

Figure~3 shows the 2e-ARPES data acquired around the Fermi level. Measurements were performed at two temperatures: 8.5~K, well below the superconducting transition temperature $T_c = 93$~K, and 200~K, far above $T_c$. The data are analyzed using the normalized correlation measure $P^{(2)}$, which quantifies the relative intensity of true coincidence events after subtraction of the uncorrelated background (Methods and Supplementary Information). The full two-electron dataset is intrinsically six-dimensional, with each coincidence event characterized by the energy and two in-plane momentum components of each electron. To visualize the correlated signal, we first integrate over momentum and plot the joint energy map $P^{(2)}(E_1,E_2)$. These joint energy maps provide an overview of how the absorbed photon energy is distributed between correlated photoelectrons.

\begin{figure*}
\centering
\includegraphics[width=18cm]{fig4_updated.pdf}
\caption{\textbf{Temperature dependence of diagonal and anti-diagonal widths in the 2e-ARPES signal.} \textbf{(a)-(c)} Contour plots of $P^{(2)}(E_1,E_2)$ at 8.5~K, 30~K and 70~K. Similarly colored lines represent contours along the same relative intensity. Diagonal cuts \textbf{(d)} and anti-diagonal cuts \textbf{(e)} of $P^{(2)}(E_1,E_2)$ at 8.5~K, 30~K and 70~K. Solid lines are Lorentzian best fits to the data. \textbf{(f)} Full width at half maximum (FWHM) extracted from Lorentzian fits to the anti-diagonal cuts. Error bars indicate the 68\% confidence interval of the Lorentzian fits from \textbf{(e)}, calculated from the uncertainties in the fitting parameters.}
\label{fig:2eARPES_linewidths}
\end{figure*}

Figure~3a reveals a striking feature at 8.5~K, with a sharp, well-defined peak in the two-electron energy distribution. The peak is centered at $E_1=E_2=0$, corresponding to zero pair-binding energy as established by conventional ARPES, with intensity concentrated along the diagonal $E_-=E_1-E_2=0$. In contrast, measurements performed at 200~K (Fig.3b) show a pronounced suppression of the correlated signal and no discernible peak is observed at zero binding energy. The presence (absence) of the zero-energy peak at 8.5~K (200~K) is also evident in the diagonal cuts of $P^{(2)}(E_1,E_2)$ shown in Fig.~3c.

The presence of a zero-energy peak in $P^{(2)}(E_1,E_2)$ below $T_c$ is a clear signature of Cooper-pair photoemission from the superconducting condensate and has been predicted to occur in previous theoretical work on double photoemission from superconductors \cite{Berakdar2003,Mahmood2022}. In particular, as first noted by \cite{Berakdar2003}, double photoemission from a superconducting state exhibits a qualitatively distinct spectral feature from single-particle photoemission: a peak at zero pair-binding energy that exists only below $T_c$. The physical origin of this distinction lies in the nature of the excitation created by the photon. In conventional photoemission, absorption of a photon leads to the ejection of an electron from a Cooper pair, which requires a binding energy of $\Delta_{\bf k}$.
In contrast, in double photoemission the photon removes both electrons from a Cooper pair simultaneously which does not break the Cooper pair and thus does not cost any binding energy, therefore producing a peak at zero energy.

To further confirm that the zero-energy peak originates from the superconducting condensate, we next examine the momentum structure of the correlated electron pairs by restricting the analysis to a narrow energy window centered around the origin in Fig.~3a. To characterize the pair momentum, we construct a pair-momentum map of $P^{(2)}$ using the same subset of coincidence events (Fig.~3d). In this representation, the horizontal and vertical axes are the center-of-mass momentum components $K_x=k_{1x}+k_{2x}$ and $K_y=k_{1y}+k_{2y}$. The resulting distribution thus provides a direct measure of the pair momentum. A pronounced maximum is observed at $\mathbf K=0$, indicating that the dominant contribution to the correlated signal arises from electron pairs with zero pair momentum, as expected for Cooper pairing in optimally doped Bi-2212 \cite{Mahmood2022,Berakdar2003}. At least for optimal doping, no signature of a pair-density wave, corresponding to a peak at non-zero $\mathbf{K}$ \cite{Mahmood2022}, is observed \cite{Agterberg2020}.

Having established the superconducting condensate-associated feature, we next examine its temperature dependence in the two-dimensional energy distribution. We consider two coordinates, the total energy $E_+=E_1+E_2$ and the relative energy $E_-=E_1-E_2$, corresponding to the diagonal and anti-diagonal directions of the joint energy map, respectively. These coordinates distinguish changes in the total detected energy from changes in how that energy is shared between the two electrons.

Figures 4(a)-(c) show the evolution of the joint energy distribution at 8.5~K, 30~K and 70~K. The most striking feature is that the width along the relative-energy direction (anti-diagonal, Fig.~4(e)) increases substantially upon cooling, whereas the width along the total-energy direction (diagonal, Fig.~4(d)) remains nearly unchanged. Lorentzian fits to the experimental cuts yield a relative-energy full width at half maximum that increases from approximately 12~meV at 70~K to 23~meV at 8.5~K, as shown in Fig.~4(f). Thus, as superconductivity strengthens upon cooling, the detected two-electron energy distribution becomes increasingly broadened in the relative-energy coordinate without a corresponding increase in its total-energy width.

This contrasting temperature dependence cannot be explained by the temperature-independent instrumental resolution nor by the thermal broadening commonly present in standard ARPES, as the latter should decrease as the temperature is lowered. Rather, it suggests that the double-photoemission process is subject to an energy redistribution that can only arise from its interaction with the collective degrees of freedom of the superconductor itself. This, in turn, would imply that the joint energy map  $P^{(2)}(E_1,E_2)$ provides unique access to excitations present inside the superconducting state.

While determining the microscopic mechanism responsible for this enhanced anti-diagonal broadening is beyond the scope of our work, we discuss two complementary scenarios. In the first one (Supplementary Information Sec.~IV), the first ejected photoelectron undergoes intermediate-state Coulomb scattering off electrons in the material before the second photoelectron is emitted. Such scattering processes transfer energy and momentum between the first photoelectron and the electronic system, thus naturally explaining the relative difference in two photo-electrons' energies. Since the second photo-electron can be subject to the same scattering processes after emission, a finite distribution of detected photoelectron energies would result. We note that these scattering processes would necessarily lead to a coupling of the photo-electrons to collective spin or charge excitations inside the superconductor \cite{Fong1999,Guarise2014,Mitrano2018}, thus directly probing its strongly corelated nature. 

A second possibility involves the relative-time dynamics of the outgoing two-electron state. In this description (Supplementary Information Sec.~V), the two high-energy electrons are initially generated with equal energy ($E_-=0$) by an effective pair-emission process. However, each outgoing electron subsequently interacts with collective excitations present in the superconducting state of the material, resulting in different scattering histories. This introduces an additional relative-time dependence into the two-electron photoemission amplitude, broadening the measured distribution of the energy difference between the electrons. Within this framework, the relative-energy linewidth reflects both the lifetime or dephasing of the outgoing electrons due to their coupling to these collective excitations. A natural source is fluctuations of the superconducting order parameter \cite{Emery1995,Corson1999, Corson_2000}, which provide a time-dependent and spatially non-uniform environment through which the two photoelectrons propagate. In the cuprates, the short coherence length, strong momentum dependence of the gap and electronic inhomogeneity \cite{Pan2001,McElroy2005,Pelc2018} can make these fluctuations particularly effective at giving the two electrons different scattering histories. As the condensate amplitude strengthens on cooling, it can overcome the suppression of the thermal excitation of these modes, producing the larger anti-diagonal linewidth observed at low temperature.

Both mechanisms illustrate how the energy distribution in double photoemission can carry information beyond the properties of the Cooper pair itself. The observation of a superconducting condensate-associated peak establishes 2e-ARPES as an experimental probe of Cooper-pair emission, while its unexpected linewidth evolution points toward a broader opportunity to investigate the interactions and dynamics accompanying pair removal in correlated materials.

\vspace{2mm}
\noindent\textbf{Acknowledgments:} We thank Peter Abbamonte, Peter Armitage, Juan C. Campuzano, Tai-Chang Chiang, Eugene Demler, Vidya Madhavan, Mike Norman, Mohit Randeria, George Sawatzky, Z.-X. Shen, and Lucas Wagner for helpful discussions. 
The work by H.A., J.Z., and F.M. was supported by the EPiQS program of the Gordon and Betty Moore Foundation, Grant GBMF11069, and by the  U.\ S.\ Department of Energy, Office of Science, Basic Energy Sciences, under Award No.\ DE-SC0021238 (project conception).
The work at BNL was supported by the U.\ S.\ Department of Energy, Office of Science, Basic Energy Sciences, Materials Sciences and Engineering Division, under contract no. DE-SC0012704. The work by K.H.W. and D.K.M was supported by the U.\ S.\ Department of Energy, Office of Science, Basic Energy Sciences, under Award No.\ DE-FG02-05ER46225.
J.N. was partly supported by the U.\ S.\ Department of Energy, Office of Science, Office for Nuclear Physics under award no.~DE-SC0023861.
The authors acknowledge the use of facilities and instrumentation supported by NSF through the University of Illinois at Urbana-Champaign Materials Research Science and Engineering Center DMR-2309037.
Sample characterization was carried out in part in the Materials Research Laboratory Central Research Facilities, University of Illinois.

\vspace{2mm}
\noindent\textbf{Author contributions:} H.A. and J.Z. performed the measurements and analyzed the experimental data. G.G. synthesized the optimally doped Bi-2212 single crystals. K.H.W. and D.K.M. performed the simulation presented in Fig.~1b and in SI Sec.I. D.K.M. developed the theoretical description of intermediate-state Coulomb scattering during double photoemission (SI Sec.~IV). R.M.F. and J.N. developed the theoretical framework relating relative-energy broadening to relative-time dynamics and dephasing of the emitted two-electron state (SI Sec.~V). All authors contributed to the writing of the manuscript. F.M. supervised the project.

\vspace{2mm}
\noindent\textbf{Competing interests:} The authors declare no competing interests.

\vspace{2mm}
\noindent\textbf{Methods}
\vspace{1mm}

\noindent \textit{Experimental setup:} Our 2e-ARPES setup uses a gas based high-harmonic generation (HHG) beamline as a photon source. A Yb:KGW laser (CARBIDE, Light Conversion) provides a 1030~nm fundamental beam with a pulse energy of 120~\(\mu\)J and a repetition rate of 525~kHz. High harmonics are generated by focusing the fundamental beam into a synthetic fused-silica hollow-core fiber waveguide (XUUS-5, KM Labs) filled with xenon gas. The resulting extreme-ultraviolet (XUV) radiation is monochromated to a photon energy of 22.8~eV, corresponding to the highest harmonic generated with appreciable flux under these conditions. The monochromated XUV beam is focused onto the sample with a spot size of 200 $\mu$m and serves as the photoemission probe for both conventional ARPES and two-electron coincidence measurements. Photoelectrons are detected using two angle-resolved time-of-flight analyzers (ARTOF-2, Scienta Omicron) positioned perpendicular to each other. The analyzers are equipped with delay-line detectors (DLD40, RoentDek) and synchronized timing circuits (TDC8HP, RoentDek). The sample temperature was controlled between 8~K and 300~K using a closed-cycle helium cryostat (ARS-4HW compressor and DE-202SB cold head, Advanced Research Systems). A six-axis manipulator (CryoArc) coupled to the cold head provided precise control of the sample position and orientation, with translational and angular resolutions of 1 $\mu$m and $10^{-3}$ rad, respectively.

\vspace{1mm}
\noindent \textit{Correlation measure:}
Each detected photoelectron is characterized by its energy $E_i$ and in-plane momentum $\mathbf{k}_i$, collectively denoted by $\xi_i=(E_i,\mathbf{k}_i)$, where $i=1,2$ labels the detector. In our 2e-ARPES measurements, $E_i$ is defined relative to the Fermi level, as determined from conventional ARPES measurements. The same-pulse coincidence distribution, $I^{(2)}(\xi_1,\xi_2)$, counts events in which one electron is detected in each analyzer following the same laser pulse. These events include true double photoemission, in which a single photon induces the emission of two electrons, and accidental coincidences arising from independent single-electron photoemission events within the same laser pulse.

For statistically independent single-electron emission, the expected accidental-coincidence distribution factorizes as
\begin{equation}
I_{\mathrm{acc}}^{(2)}(\xi_1,\xi_2)
=
I^{(1)}(\xi_1)I^{(1)}(\xi_2),
\end{equation}
where $I^{(1)}(\xi_i)$ denotes the single-electron intensity, normalized such that its product gives the expected number of accidental coincidences. Experimentally, $I_{\mathrm{acc}}^{(2)}$ is estimated by pairing electrons detected in different laser pulses, as described below. Because electrons from different pulses cannot originate from the same microscopic emission event, this provides a direct estimate of the uncorrelated background.

We define the two-electron correlation measure
\begin{equation}
P^{(2)}(\xi_1,\xi_2)
=
\frac{
\left[
I^{(2)}(\xi_1,\xi_2)
-
I_{\mathrm{acc}}^{(2)}(\xi_1,\xi_2)
\right]^2
}{
I^{(2)}(\xi_1,\xi_2)
+
I_{\mathrm{acc}}^{(2)}(\xi_1,\xi_2)
+
\epsilon
},
\label{eq:P2}
\end{equation}
where $\epsilon>0$ is a small regularization parameter that stabilizes bins containing very few counts. The numerator represents the squared coincidence excess above the accidental background, while the denominator provides a normalization based on the total counting intensity. Thus, $P^{(2)}$ characterizes the strength of correlations beyond those expected from independent photoemission. The features analyzed in this work correspond to a positive excess of same-pulse coincidences before the difference is squared. Further details of the pulse-offset subtraction and the connection between the coincidence rate and the two-electron photoemission probability are provided in the Supplementary Information.

\vspace{1mm}
\noindent\textit{Coincidence data analysis:}

Photoelectrons were recorded using two angle-resolved time-of-flight analyzers, synchronized to the laser repetition clock. Each detection event was assigned a laser-pulse index $n$, allowing electron pairs to be identified according to their pulse of origin.

For each energy- and momentum-resolved bin $(\xi_1,\xi_2)$, we construct the pulse-offset coincidence histogram:
\begin{equation}
M_l(\xi_1,\xi_2)
=
\sum_n
c_{1,n}(\xi_1)c_{2,n-l}(\xi_2),
\label{eq:alg}
\end{equation}
where $c_{i,n}(\xi_i)$ equals one when detector $i$ records exactly one electron in bin $\xi_i$ from pulse $n$, and zero otherwise. The integer $l$ denotes the pulse offset between the two detectors, with the sum restricted to valid pulse indices.

The measured same-pulse coincidence distribution is
\begin{equation}
I^{(2)}(\xi_1,\xi_2)=M_0(\xi_1,\xi_2).
\end{equation}
The accidental-coincidence distribution is estimated by averaging the histograms obtained from the two nearest-neighbor pulse offsets:
\begin{equation}
I_{\mathrm{acc}}^{(2)}(\xi_1,\xi_2)
=
\frac{
M_{+1}(\xi_1,\xi_2)
+
M_{-1}(\xi_1,\xi_2)
}{2}.
\end{equation}

Because the detected electron time-of-flight window is shorter than the laser repetition period, electrons assigned to different pulses cannot originate from the same microscopic photoemission event. Provided that the pulse-to-pulse detection statistics are stationary and independent, the offset histograms therefore estimate the accidental background. The correlation measure $P^{(2)}(\xi_1,\xi_2)$ is then calculated using Eq.~\ref{eq:P2}. Additional experimental checks and details of the background estimation are provided in the Supplementary Information.

\vspace{1mm}
\noindent \textit{Bootstrapping:}
Statistical uncertainties in \(P^{(2)}\) are estimated using bootstrap resampling \cite{Bootstrap_intro_new}.
The same-pulse and pulse-offset coincidence samples are resampled independently with replacement.
For each bootstrap realization, the distributions
\(I^{(2)}(\xi_1,\xi_2)\) and
\(I_{\mathrm{acc}}^{(2)}(\xi_1,\xi_2)\)
are reconstructed, and the corresponding
\(P^{(2)}(\xi_1,\xi_2)\)
is calculated using Eq.~\ref{eq:P2}.
This procedure is repeated to generate a bootstrap distribution of \(P^{(2)}\) in each \((\xi_1,\xi_2)\) bin.
The standard deviation of this distribution is taken as the statistical uncertainty.
Further details are provided in the Supplementary Information.

\vspace{2mm}
\noindent\textbf{Data availability:} The data in this manuscript are available from the corresponding author upon reasonable request.

\vspace{2mm}
\noindent\textbf{Corresponding author:} Correspondence to Fahad Mahmood~(fahad@illinois.edu).
